A complete description of thermodynamic stabilities of molecular crystals

Predictions of relative stabilities of (competing) molecular crystals are of great technological relevance, most notably for the pharmaceutical industry. However, they present a long-standing challenge for modeling, as often minuscule free energy differences are sensitively affected by the description of electronic structure, the statistical mechanics of the nuclei and the cell, and thermal expansion. The importance of these effects has been individually established, but rigorous free energy calculations for general molecular compounds, which simultaneously account for all effects,have hitherto not been computationally viable. Here we present an efficient "end to end" frame-work that seamlessly combines state-of-the art electronic structure calculations, machine-learning potentials, and advanced free energy methods to calculate ab initio Gibbs free energies for general organic molecular materials. The facile generation of machine-learning potentials for a diverse set of polymorphic compounds, benzene, glycine, and succinic acid, and predictions of thermodynamic stabilities in qualitative and quantitative agreement with experiments highlights that predictive thermodynamic studies of industrially-relevant molecular materials are no longer a daunting task.

==> preamble.tex <==
\usepackage[english]{babel}
%\usepackage[utf8x]{inputenc}
%\usepackage[colorinlistoftodos, color=green!40, prependcaption]{todonotes}
\usepackage{xcolor}

%\usepackage[pdftex, pdftitle={Article}, pdfauthor={Author}]{hyperref} % For hyperlinks in the PDF
%\setlength{\marginparwidth}{2.5cm}


\usepackage{amsthm}
\usepackage{mathtools}
\usepackage{physics}
\usepackage{graphicx}
%\usepackage[left=23mm,right=13mm,top=35mm,columnsep=15pt]{geometry} 
\usepackage{adjustbox}
\usepackage{placeins}
\usepackage[T1]{fontenc}
\usepackage{lipsum}
\usepackage{csquotes}
\usepackage{soul}

% SI
\newcommand{\si}{Supplemental Information}
% comments
%\newcommand{\todos}[1]{{\color{red}{#1}}}
\newcommand{\eae}[1]{{\color{blue} #1}}
\newcommand{\vk}[1]{{\color{purple} #1}}

\renewcommand{\eae}[1]{{\color{black} #1 }}
\renewcommand{\vk}[1]{{\color{black} #1 }}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand*{\Ang}{\, \mbox{\normalfont\AA}} % Angstrom
\newcommand{\JmolK}{\, \mathrm{J} \mathrm{mol}^{-1} \mathrm{K}^{-1}} % J mol^-1 K^-1
\newcommand{\eV}{\, \mathrm{eV}} % eV
\newcommand*{\meV}{\, \textrm{meV}}
\newcommand*{\meVsa}{\, \textrm{meV}/\textrm{\AA}^2}
\newcommand*{\kJmol}{\, \textrm{kJ/mol}}
\newcommand*{\Jmol}{\, \textrm{J/mol}}
\newcommand*{\kcalmol}{\, \textrm{kcal/mol}}
\newcommand*{\calmol}{\, \textrm{cal/mol}}
\newcommand*{\Vesta}{\textsc{Vesta}}
\newcommand*{\invcm}{\, \textrm{cm}^{-1}}
% math notations
\newcommand{\avg}[1]{\ensuremath{\left<#1\right>}}
\newcommand{\pd}[2]{\ensuremath{\frac{\partial {#1}}{\partial {#2}}}}
\newcommand{\pds}[2]{\ensuremath{\frac{\partial^2 {#1}}{\partial {#2}}}}
\newcommand{\bigo}[1]{\ensuremath{\mathcal{O}\left({#1}\right)}}
\newcommand{\D}{\ensuremath{\mathrm{d}}}
% thermodynamics symbols
\newcommand{\tm}{\ensuremath{T_{\text{m}}}} %
\newcommand{\kb}{k_{\rm B}} %
% Hamiltonians 
\newcommand{\hdft}{\ensuremath{\mathcal{H}}} %
\newcommand{\hml}{\ensuremath{\mathcal{H}_{\text{MLP}}}} %
\newcommand{\hdebye}{\ensuremath{\mathcal{H}_{\text{Debye}}}} %
\newcommand{\hdftcl}{\ensuremath{\mathcal{H}^{\text{cl}}}} %
\newcommand{\hmlcl}{\ensuremath{\mathcal{H}_{\text{MLP}}^{\text{cl}}}} %
\newcommand{\hdebyecl}{\ensuremath{\mathcal{H}_{\text{Debye}}^{\text{cl}}}} %
% potentials and free energies
\newcommand{\udft}{\ensuremath{U}} %
\newcommand{\uml}{\ensuremath{U_{\text{MLP}}}} %
\newcommand{\umlhar}{\ensuremath{U_{\text{MLP}}^{\text{har}}}} %
\newcommand{\gdft}{\ensuremath{G}} %
\newcommand{\gml}{\ensuremath{G_{\text{MLP}}}} %
\newcommand{\gdftcl}{\ensuremath{G^{\text{cl}}}} %
\newcommand{\gmlcl}{\ensuremath{G_{\text{MLP}}^{\text{cl}}}} %
\newcommand{\gdebyecl}{\ensuremath{G_{\text{Debye}}^{\text{cl}}}} %
\newcommand{\adft}{\ensuremath{A}} %
\newcommand{\aml}{\ensuremath{A_{\text{MLP}}}} %
\newcommand{\adftcl}{\ensuremath{A^{\text{cl}}}} %
\newcommand{\amlcl}{\ensuremath{A_{\text{MLP}}^{\text{cl}}}} %
\newcommand{\adfthar}{\ensuremath{A^{\text{har}}}} %
\newcommand{\amlhar}{\ensuremath{A_{\text{MLP}}^{\text{har}}}} %
\newcommand{\adebyecl}{\ensuremath{A_{\text{Debye}}^{\text{cl}}}} %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\ficm}{\ensuremath{\Tilde{m}}} %






